Large Language Models as Annotators: Enhancing Generalization of NLP Models at Minimal Cost

State-of-the-art supervised NLP models achieve high accuracy but are also susceptible to failures on inputs from low-data regimes, such as domains that are not represented in training data. As an approximation to collecting ground-truth labels for the specific domain, we study the use of large language models (LLMs) for annotating inputs and improving the generalization of NLP models. Specifically, given a budget for LLM annotations, we present an algorithm for sampling the most informative inputs to annotate and retrain the NLP model. We find that popular active learning strategies such as uncertainty-based sampling do not work well. Instead, we propose a sampling strategy based on the difference in prediction scores between the base model and the finetuned NLP model, utilizing the fact that most NLP models are finetuned from a base model. Experiments with classification (semantic similarity) and ranking (semantic search) tasks show that our sampling strategy leads to significant gains in accuracy for both the training and target domains.

==> tables/amazon_books_ood.tex <==
\begin{table}[h]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
 & OOD Train & OOD Test\\
\hline
Std & 14.49 & 17.37\\
\hline
Std + Real Easiest 40\% & 17.18 & 18.33 \\
Std + Real Middle 40\%  & 18.52 & 18.30\\
Std + Real Hardest 40\%  & 20.04 & 18.59\\
Std + Real Uniform 40\%  & 18.41 & 18.22 \\
\hline
Std + GPT Easiest 40\% & 15.00 & 18.06 \\
Std + GPT Middle 40\%  & 16.39 & 18.33 \\
Std + GPT Hardest 40\%  & 16.63 & 17.95 \\
Std + GPT Uniform 40\%  & 15.86 & 18.28 \\

\hline
\end{tabular}
}
\caption{\label{tab:amazon_books_ood}
Amazon Books P@1 on different sets. GPT Annotations are good for all examples}
% \vspace*{-15pt}
\end{table} 


==> tables/old_quora_ood_table.tex <==
\begin{table}[h]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|ll|}
\hline
& Complete AUC  & AUC on Hard 30\% & AUC on Easy 30\% \\
\hline
Complete & 91.01 & 80.65 & 98.01\\
Hard 30\% Removed & 86.46 & 55.95 & -\\
Hard 30\% Removed 30 \% GPT Aug & 87.99 & 63.42& - \\
Hard 30\% Removed 10 \% GPT Aug & 87.89 & 61.49 & - \\
Easy 30\% Removed  & 89.70 & - & 96.36 \\
Easy 30\% Removed 30 \% GPT Aug & 89.42 & - & 96.43 \\
Easy 30\% Removed 10 \% GPT Aug & 89.54 & - & 96.30 \\
\hline
\end{tabular}
}
\caption{%\label{tab:quora_ood_hardveasy}
Quora GPT Annotations are good for Hard examples and not for Easy examples}
% \vspace*{-15pt}
\end{table} 


==> tables/quora_ood_hardveasy.tex <==
% \begin{table}[h]
% \centering
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{|l|ll|}
% \hline
% & OOD   & Total \\
% \hline
% ID set & 51.392 $\pm$ 0.105 & 54.561 $\pm$ 0.158 \\
% \hline
% ID set + Random 10\% LLM & 54.828 $\pm$ 0.244 & 58.389 $\pm$ 0.208\\
% ID set + Uncertain 10\% LLM & 53.627 $\pm$ 0.238 & 56.871 $\pm$ 0.202 \\
% ID set + Cheat Hard 10\% LLM & 55.496 $\pm$ 0.293 & 58.911 $\pm$ 0.268 \\
% ID set + Hard 10\% LLM & 53.084 $\pm$ 0.239 & 56.444 $\pm$ 0.275 \\
% % ID set + OOD GT 30\% Uniform & 89.18 & 90.05  \\
% % ID set + OOD GT 30\% Easy & 83.36 & 86.20\\
% % ID set + OOD GT 30\% Hard  & 89.26 & 89.66\\
% \hline
% ID set + Random 10\% GT & 56.589 $\pm$ 0.213 & 59.898 $\pm$ 0.243\\
% ID set + Uncertain 10\% GT & 54.520 $\pm$ 0.197 & 57.474 $\pm$ 0.236 \\
% ID set + Cheat Hard 10\% GT & 58.175 $\pm$ 0.726 & 60.710 $\pm$ 0.758 \\
% ID set + Hard 10\% GT & 54.482 $\pm$ 0.275 & 57.113 $\pm$ 0.376 \\
% % ID set + OOD LLM 30\% Uniform  & 85.56 & 87.49 \\
% % ID set + OOD LLM 30\% Easy  & 85.17 & 87.10 \\
% % ID set + OOD LLM 30\% Hard  & 86.91 & 88.40 \\
% \hline
% \end{tabular}
% }
% \caption{\label{tab:quora_ood_hardveasy}
% Quora GPT Annotations are good for Hard examples and not for Easy examples}
% % \vspace*{-15pt}
% \end{table} 


==> tables/wikipedia_usa_ood.tex <==
\begin{table}[h]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|l|lH|}
\hline
 & OOD Train & OOD Test & Complete\\
\hline
% Complete & 29.57 & 12.54 (44.33) & 19.09\\
% Real Easiest 40\% & 35.91 & 13.56 (49.42) & 19.31\\
% Real Middle 40\%  & 39.83 & 13.99 (50.30) & 19.37\\
% Real Hardest 40\%  & 40.18 & 13.89 (48.77) & 19.40\\
% Real Uniform 40\%  & 39.29 & 14.13 (50.82) & 19.36\\
% GPT Easiest 40\% & 32.42 & 13.23 (47.00) & 19.26\\
% GPT Middle 40\%  & 33.09 & 13.21 (46.81) & 19.23\\
% GPT Hardest 40\%  & 32.34 & 13.36 (47.53) & 19.15\\
% GPT Uniform 40\%  & 32.84 & 12.95 (45.84) & 19.17\\

Std & 29.57 & 12.54 & 19.09\\
\hline
Std + Real Easiest 40\% & 35.91 & 13.56 & 19.31\\
Std + Real Middle 40\%  & 39.83 & 13.99  & 19.37\\
Std + Real Hardest 40\%  & 40.18 & 13.89 & 19.40\\
Std + Real Uniform 40\%  & 39.29 & 14.13 & 19.36\\
\hline
Std + GPT Easiest 40\% & 32.42 & 13.23 & 19.26\\
Std + GPT Middle 40\%  & 33.09 & 13.21 & 19.23\\
Std + GPT Hardest 40\%  & 32.34 & 13.36 & 19.15\\
Std + GPT Uniform 40\%  & 32.84 & 12.95 & 19.17\\

\hline
\end{tabular}
}
\caption{\label{tab:wikipedia_usa_ood}
Wikipedia P@1 on different sets. GPT Annotations are good for Hard examples and not for Easy examples}
% \vspace*{-15pt}
\end{table} 

